On Occlusions in Video Action Detection: Benchmark Datasets And Training Recipes

This paper explores the impact of occlusions in video action detection. We facilitate this study by introducing five new benchmark datasets namely O-UCF and O-JHMDB consisting of synthetically controlled static/dynamic occlusions, OVIS-UCF and OVIS-JHMDB consisting of occlusions with realistic motions and Real-OUCF for occlusions in realistic-world scenarios. We formally confirm an intuitive expectation: existing models suffer a lot as occlusion severity is increased and exhibit different behaviours when occluders are static vs when they are moving. We discover several intriguing phenomenon emerging in neural nets: 1) transformers can naturally outperform CNN models which might have even used occlusion as a form of data augmentation during training 2) incorporating symbolic-components like capsules to such backbones allows them to bind to occluders never even seen during training and 3) Islands of agreement can emerge in realistic images/videos without instance-level supervision, distillation or contrastive-based objectives2(eg. video-textual training). Such emergent properties allow us to derive simple yet effective training recipes which lead to robust occlusion models inductively satisfying the first two stages of the binding mechanism (grouping/segregation). Models leveraging these recipes outperform existing video action-detectors under occlusion by 32.3% on O-UCF, 32.7% on O-JHMDB & 2.6% on Real-OUCF in terms of the vMAP metric. The code for this work has been released at https://github.com/rajatmodi62/OccludedActionBenchmark.

==> sections/discussions.tex <==
\section{Discussion}



% \textbf{Enhancing Natural robustness:} It can be worthwhile to explore how to devise architectures which can be naturally robust \textit{without depending} on the pre-trained weights. For applications like biomedical image segmentation, relevant in-domain large-scale datasets might not be available for pre-training.  
% Three  troubling questions naturally arise. \textbf{What happens when the number of capsules are less than the objects in videos?}
% We observe that a single capsule starts representing multiple occluders even if they represent different wholes. On the other-hand a parse-tree expects a single root while representing an object \cite{hinton2021represent}. Each parse-tree must be unique and separately converged to for \textit{each unique} object instance rather than a single capsule mixing multiple such trees together. Secondly, while a capsule represents objects, the relationships among different objects are not modelled. That is a question for scene representations\cite{mildenhall2021nerf}, but can't be answered by simple rendering.  

% \textbf{Can capsules generalize to detecting/tracking objects not seen during training?} A  limitation of capsules is that they bind to a specific object [eg,human],which prevents a finite number of capsules from representing a large number of objects which don't share common parts. Recent works on reusable slots \cite{locatello2020object}, binds a slot to \texit{any} object without loss of this generality. We hope to explore if such slots can represent \textit{each occluder} (and occludee) separately using  only minor supervision (eg, optical flow) \cite{kipf2021conditional}.

% \textbf{Can capsules specialize between occluder/occludees?} In Fig \ref{fig:separation} we show that capsules are able to achieve separation between occluder and object regions, even when \textit{no  segmentation mask of occluders} is present during training. A possible direction is to separate object/occludee level capsules into two separate routing streams \cite{simonyan2014two} and then have them compete to explain the presence of an occluder at a particular pixel \cite{kortylewski2019localizing}.


 

==> supp_figs/instance.tex <==

\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/instance_1.pdf}
    % \vspace{-5mm} 
    \caption{\textbf{Our instance-level annotations for UCF-24:} We propose a new benchmark of instance-level action segmentation and release official annotations.
    }\label{fig:instance_1}
    \vspace{-5mm}
\end{figure}

\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/instance_2.pdf}
    % \vspace{-5mm} 
    \caption{ \textbf{Our instance-level annotations for UCF-24:} We propose a new benchmark of instance-level action segmentation and release official annotations.
    }\label{fig:instance_2}
    \vspace{-5mm}
\end{figure}


==> supp_figs/real_data.tex <==

\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/d1.pdf}
    % \vspace{-5mm} 
    \caption{ \textbf{Our Real-OUCF:} contains realistic occlusions with instance-level action annotations.
    }\label{fig:real_1}
    \vspace{-5mm}
\end{figure}

\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/d2.pdf}
    % \vspace{-5mm} 
    \caption{ \textbf{Our Real-OUCF:} contains realistic occlusions with instance-level action annotations.
    }\label{fig:real_2}
    \vspace{-5mm}
\end{figure}


==> supp_figs/synth.tex <==

\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/synth_1.pdf}
    % \vspace{-5mm} 
    \caption{ \textbf{Different occluder trajectories:} are illustrated for our proposed O-UCF and O-JHMDB datasets.
    }\label{fig:synth_1}
    \vspace{-5mm}
\end{figure}


\begin{figure}[t]
    \centering
    %\vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{supp_figs/synth_2.pdf}
    % \vspace{-5mm} 
    \caption{ \textbf{Nature of Occluders}: Occluders in the proposed O-UCF \& O-JHMDB datasets belong to either indoor/outdoor samples. 
    }\label{fig:synth_2}
    \vspace{-5mm}
\end{figure}

==> supp_sections/intro.tex <==
\section{Introduction}

==> supp_sections/representational_collapse.tex <==
\subsection{Representational Collapse in Capsules}
\label{sec:rep_collapse}
In Fig 5 of the main manuscript, we have shown the problem of representational collapse\footnote{This section is meant to be philosophical and optimistic in nature. The kind reader is requested to skip it if concrete-results are desired.},  where capsules cannot decode multiple entities (objects), if the number of objects in the scene are greater than the parameters in the network. A classical way to solve this problem would be to to increase the number of parameters by reinitializing and retraining the machine again. It agrees with the evolutionary observation that more parameters mean more intelligence and the only option to do better is to scale up (i.e 85 billion neurons in the brain vs 100 trillion in ChatGPT4). This is a promising direction if we want to continue to pay exorbitant amounts of money for specialist hardware, expensive electricity or wait for the hardware to become cheaper in future. 

\textbf{Mortal computation requires self-replicable embeddings:} On the other hand if we want to pack similar levels of intelligence in a brain-like interface which consumes less than 25 watts daily, we have to take an alternate biologically-plausible route\cite{hinton2022represent}: intelligence can be encoded in a single cell (embedding) much like how the genetic code of a human gets encoded in the DNA. In nature, multiple copies of a zygote (cell) lead to emergence of an animal's internal organs. Similarly, in our computers multiple copies of this single replicable embedding shall lead to networks whose structure gets discovered 'on-the-fly' according to local hardware constraints. 

It has been well established in Distillation literature that \cite{hinton2015distilling} a higher-parameterized teacher network can teach a lower-parameter student network to obtain similar performance. If all the knowledge of the teacher could be compressed into a singular embedding, then we won't need distillation at all. Simply copying the single embedding many times on  a weaker student hardware would be enough to allow the student model to exist. These 'connectionist-networks'\cite{hinton1990connectionist} which start their existence from a single embedding and only remain in the memory as long as the hardware is powered on (hence the name mortal) would require  learning algorithms other than backpropogation: where the parameters of each layer could be updated without knowing the precise feed-forward mathematical-functions\cite{hinton2022forward} and allow dynamic growing of the network on a smaller hardware\cite{jia2016dynamic}. 


We are very excited to see how this direction turns out for our community. 



==> supp_sections/sota.tex <==
\subsection{A Robust Video-Level State Of The Art}
\label{sec:sota}
We present a new state-of-the-art in spatio-temporal video action detection specifically on UCF-24 and JHMDB-21 datasets in Tab\ref{tab:sota}. Note that we achieve 83.1\% on UCF-24 and 98.1\% on JHMDB-21 in terms of the widely accepted\cite{kalogeiton2017action} v-mAP metric at the 0.5ioU threshold. One of the most desirable properties in an action-detector is that it should perform well on \textit{existing} standard datasets\cite{soomro2012ucf101} as well as be \textit{robust to occlusions} at the same time. Our simple model namely VCAPS-Mvitv2 achieves the best of both worlds, thereby setting a new video-level state of the art for our community.

The robustness of an action-detector can be measured in two ways, 1) the \textit{actual robustness} under occlusions which has been illustrated  as absolute value (i.e. 67.3\%) in Tab6 of our original manuscript. 2) Measuring the drop in performance of a detector as the ioU threshold during evaluation is swept from $0.2$ to $0.5$. We define this quantity as $\kappa = 1- (\frac{vmAP_{0.2}- vmAP_{0.5}}{vmAP_{0.2}})$ which simply measures the relative performance drop from 0.2$\rightarrow$0.5ioU. In Tab\ref{tab:sota}, we note that on the much challenging UCF-24 dataset, our method obtains $\kappa= 0.84$, which is greater than all the other methods, thereby indicating more localization robustness. On JHMDB-21, we obtain 92.8\% in terms of the absolute v-mAP score, which is significantly better than other existing methods. We acknowledge that TubeR\cite{zhao2022tuber} and ST-Mixer \cite{wu2023stmixer} are slightly better than our method in terms of f-mAP scores on UCF-24 dataset, although our method is considerably \textit{more} robust (0.84 vs 0.71 on $\kappa$ score).

\input{supp_tab/sota}

==> supp_tab/sota.tex <==
\begin{table}[!htbp]
\caption{\textbf{Comparison with existing methods:} Comparison of our method across existing supervised approaches, *: denotes results using a CSN152 backbone. $\kappa = 1- (\frac{vmAP_{0.2}- vmAP_{0.5}}{vmAP_{0.2}})$. Higher value of $\kappa$ denotes more robustness.}. 
\vspace{-0.4em}
% \setlength{\tabcolsep}{2pt}
\begin{center}
\begin{tabular}{c|cc|cccc|cccc}
                        &               &              & \multicolumn{4}{c|}{UCF-24}                                    & \multicolumn{4}{c}{JHMDB-21}                                  \\
\midrule
                        & \multicolumn{2}{c|}{Backbone} & f-mAP         & \multicolumn{2}{c}{v-mAP}     &        & f-mAP         & \multicolumn{2}{c}{v-mAP}     &         \\
       Methods                 & 2D            & 3D           & 0.5           & 0.2           & 0.5           &     $\kappa$           & 0.5           & 0.2           & 0.5           &      $\kappa$          \\
\midrule
\textit{Yang et al.}\cite{kalogeiton17iccv}             &     \checkmark          &              & 75.0          & 76.6          & -             & -             & -             & -             & -             & -             \\
\textit{Li et al.}\cite{li2020actions}      &    \checkmark              &              & 78.0          & 82.8          & 53.8          & 0.65          & 70.8          & 77.3          & 70.2          & 0.91          \\
\textit{Kopuklu et al.}\cite{kopuklu2019you} &      \checkmark            &      \checkmark           & 80.4          & 75.8          & 48.8          & 0.64          & 75.7          & 88.3          & 85.9          & 0.97          \\
\textit{Zhao et al.}\cite{zhao2022tuber}    &               &       \checkmark          & \textbf{81.3} & 85.3          & 60.2          & 0.71          & 82.3*         & 81.8          & 80.7          & \textbf{0.99} \\
\textit{Duarte et al.}\cite{duarte2018videocapsulenet}  &               &      \checkmark           & 78.6          & 97.1          & 80.3          & 0.83          & 64.6          & 95.1          & -             & -             \\
\textit{Kumar et al.}\cite{kumar2022end}   &               &     \checkmark            & 69.2          & 95.3          & 71.9          & 0.75          & 68.1          & 96.8          & 68.4          & 0.71          \\
\textit{Tao et al.}\cite{wu2023stmixer}     &               &       \checkmark          & \textbf{83.7} & -             & -             & -             & 86.7          & -             & -             & -             \\
\midrule
\textit{Ours}           &               &    \checkmark             & 81.2          & \textbf{98.6} & \textbf{83.1} & \textbf{0.84} & \textbf{93.0} & \textbf{98.1} & \textbf{92.8} & 0.95         \\
\bottomrule
\end{tabular}
\label{tab:sota}

\end{center} 
\vspace{-1em}
\end{table}



==> tab/bench_big_table.tex <==
\begin{table}[t]\footnotesize%\scriptsize
    \caption{Our lovely benchmark }\label{tab:bench_big}
    \setlength{\tabcolsep}{2pt}
    \begin{subtable}[t]{.9\linewidth}%\centering
    \caption{O-UCF}
        \label{tab:bench_ucf_big}
    \input{tab/bench_ucf_static_big}
        \end{subtable}
    \hfill
    \begin{subtable}[t]{.9\linewidth}%\centering
    \caption{O-JHMDB}
        \label{tab:bench_jhmdb_big}
    \input{tab/bench_jhmdb_dynamic_big}
        \end{subtable}
\vspace{-1.5em}
\end{table}

==> tab/bench_param_size.tex <==

\begin{tabularx}{\linewidth}{c|c|c|cc|cc}

% \toprule
      &           &                                                        & \multicolumn{2}{c|}{UCF} & \multicolumn{2}{c}{JHMDB} \\
      & Backbone  & \begin{tabular}[c]{@{}c@{}}\#Params\\ (M)\end{tabular} & Clean       & Occ       & Clean        & Occ        \\
\midrule
      & Resnet18 \cite{he2016deep} & 11.7                                                   &     44.7        & 26.9      &       66.1       & 51.8       \\
YOWO \cite{kopuklu2019you} & Resnet50 \cite{he2016deep} & 26                                                     &        47.4     & 28.9      &        68.7      & 54.2       \\
      & Resnet101\cite{he2016deep} & 44.6                                                   &    47.7         & 29.8      &   69.5           & 55.5       \\
\midrule
      & Resnet18 \cite{he2016deep} & 11.7                                                   & 57.7        & 36.1      & 35.2         & 18.3       \\
VCAPS \cite{duarte2018videocapsulenet}& Resnet50\cite{he2016deep}  & 26                                                     & 58.0        & 37.7      & 40.2         & 18.8       \\
      & Resnet101 \cite{he2016deep}& 44.6                                                   & 59.4        & 38.9      & 45.7         & 22.2    \\
\bottomrule
\end{tabularx}


==> tab/bench_side_by_side.tex <==

%puts motion & w/aug tables side by side. 
\begin{table}[t]\footnotesize%\scriptsize
    \caption{Our lovely benchmark }\label{tab:bench_side_by_side}
    \setlength{\tabcolsep}{2pt}
    \begin{subtable}[t]{.5\linewidth}%\centering
    \caption{O-UCF}
        \label{tab:toy_motion}
    \input{tab/bench_toy_static_dynamic}
        \end{subtable}
    \hfill
    \begin{subtable}[t]{.5\linewidth}%\centering
    \caption{O-JHMDB}
        \label{tab:bench_aug}
    \input{tab/bench_aug}
        \end{subtable}
\vspace{-1.5em}
\end{table}

==> tab/bench_static.tex <==

\begin{tabularx}{\linewidth}{c|cccc|cccc}
% \toprule
            & \multicolumn{4}{c|}{UCF}    & \multicolumn{4}{c}{JHMDB}  \\
% \midrule
            & Clean & FG1  & FG2  & FG3  & Clean & FG1  & FG2  & FG3  \\
\midrule
MOC-Clean\cite{li2020actions}   & 54.4  & 53.6 & 35.2 & 29.5 & 77.2  & 45.2 & 33.9 & 25.9 \\
YOWO-Clean \cite{kopuklu2019you} & 48.8  & 38.5 & 32.5 & 26.8 & 85.7  & 50.5 & 47.7 & 46.2 \\
VCAPS-Clean \cite{duarte2018videocapsulenet}& 75.5  & 51.5 & 42.8 & 36.9 & 65.7  & 49.2 & 35.4 & 21.7 \\
\bottomrule
% \vspace{0.5em}
\end{tabularx}


==> tab/bench_weight_analysis.tex <==

\begin{tabularx}{\linewidth}{c|cc|cc}
% \toprule
               & \multicolumn{2}{c|}{UCF} & \multicolumn{2}{c}{JHMDB} \\
               & w/o        & w          & w/o         & w           \\
\midrule
MOC   \cite{li2020actions}          & 7.4        & 39.8       & 20.7        & 35.3        \\
YOWO \cite{kopuklu2019you}         & 14.4       & 31.2       & 53.0        & 63.7        \\
VCAPS (i3D)\cite{duarte2018videocapsulenet}    & 24.2       & 42.2       & 34.5        & 35.6        \\
\hline
VCAPS (Mvitv2) & 16.8       & 67.3       & 31.8        & 86.8  \\
\bottomrule
\end{tabularx}


==> tab/benchmark.tex <==
% full benchmark dumped foolishly
%motion (toy experiments)| static severity 
\begin{table}[t]\footnotesize%\scriptsize
    \caption{Our lovely benchmark }\label{tab:bench_1}
    \setlength{\tabcolsep}{1pt}
    \begin{subtable}[t]{.49\linewidth}%\centering
    \caption{3D backbones are better under dynamic occlusions, whereas 2D backbones are better under static occlusions. }
        \label{tab:bench_motion}
    \input{tab/bench_toy_static_dynamic}
        \end{subtable}
    \hfill
    \begin{subtable}[t]{0.49\linewidth}\centering
    \caption{Increasing foreground occlusion severity reduces performance. }
    \label{tab:bench_severity}
    \input{tab/bench_static}
    \end{subtable}
\vspace{-1.5em}
\end{table}


% w & w/o Aug| w & w/o Weights
\begin{table}[t]\footnotesize%\scriptsize
    \caption{Our lovely benchmark}\label{tab:bench_2}
    \setlength{\tabcolsep}{1pt}
    \begin{subtable}[t]{.59\linewidth}%\centering
    \caption{Transformers outperform models trained even using occlusion as a data augmentation. }
        \label{tab:bench_aug}
    \input{tab/bench_aug}
        \end{subtable}
    \hfill
    % \begin{subtable}[t]{0.39\linewidth}\centering
    % \caption{Pre-trained weights improve occlusion robustness. }
    % \setlength{\tabcolsep}{2pt}
    % \label{tab:bench_weight}
    % \input{tab/bench_weight_analysis}
    % \end{subtable}
\vspace{-1.5em}
\end{table}

% diff backbones | diff param size in same model family 

\begin{table}[t]\footnotesize%\scriptsize
    \caption{Our lovely benchmark }\label{tab:bench_3}
    \setlength{\tabcolsep}{1pt}
    \begin{subtable}[t]{.49\linewidth}%\centering
    \caption{Transformers outperform other backbones with half number of parameters.}
        \label{tab:bench_backbone}
    \input{tab/bench_diff_bbns}
        \end{subtable}
    \hfill
    % \begin{subtable}[t]{0.45\linewidth}\centering
    % \caption{Increasing parameter size in the same model family increases occlusion robustness.}
    % \setlength{\tabcolsep}{1pt}
    % \label{tab:bench_parameter}
    % \input{tab/bench_param_size}
    % \end{subtable}
\vspace{-1.5em}
\end{table}

==> tab/tab_real_data.tex <==
\begin{tabularx}{\linewidth}{c|c}
                   & RealOccUcf \\

\midrule
\#Classes            & 24         \\
\#Test Videos        & 1743       \\
\#Total Instances & 20916     \\
\#No of Frames & 435749 \\
\bottomrule
\end{tabularx}

==> tab/tab_semi_real_data.tex <==

\begin{wraptable}{R}{}
\caption{A wrapped table going nicely inside the text.}\label{tab:dataset_stats}
\begin{tabularx}{0.3\linewidth}{c|cc|cc}
\multicolumn{1}{l}{} & \multicolumn{2}{c|}{OccUCF} & \multicolumn{2}{c}{OccJHMDB} \\
\multicolumn{1}{l}{} & Train       & Test      & Train        & Test       \\
\midrule
\#Severity Levels      & 9           & 9         & 9            & 9          \\
\#Occluder Motion      & 4           & 2         & 4            & 2          \\
\#Videos Per Occ       & 2284        & 923       & 660          & 268        \\
\#Total Videos         & 593840      & 20306     & 343200       & 5896 \\
\bottomrule 
\end{tabularx}
\end{wraptable} 
